Mahi-Mahi: Low-Latency Asynchronous BFT DAG-Based Consensus

We present Mahi-Mahi, the first asynchronous BFT consensus protocol that achieves sub-second latency in the WAN while processing over 100,000 transactions per second. We accomplish this remarkable performance by building Mahi-Mahi on an uncertified structured Directed Acyclic Graph (DAG). By forgoing explicit certification, we significantly reduce the number of messages required to commit and minimize CPU overhead associated with certificate verification. Mahi-Mahi introduces a novel commit rule that allows committing multiple blocks in each DAG round, while ensuring liveness in the presence of an asynchronous adversary. Mahi-Mahi can be parametrized to either attempt to commit within 5 message delays, maximizing the probability of commitment under a continuously active asynchronous adversary, or within 4 message delays, which reduces latency under a more moderate and realistic asynchronous adversary. We demonstrate the safety and liveness of Mahi-Mahi in a Byzantine context. Subsequently, we evaluate Mahi-Mahi in a geo-replicated setting and compare its performance against state-of-the-art asynchronous consensus protocols, showcasing Mahi-Mahi's significantly lower latency.

==> Makefile <==
.PHONY: FORCE lenny all clean distclean

FILE=main

all: $(FILE).pdf

%.pdf: %.tex FORCE
	latexmk -pdf $<

%.ps: %.tex FORCE
	latexmk -ps $<

clean:
	for ext in aux dvi log toc lof lot lol dlog bbl \
		nav snm fls vrb blg out tpt fdb_latexmk; \
	do \
		$(RM) $(FILE).$$ext ; \
	done
	$(RM) *.aux *.bak *~

distclean: clean
	$(RM) $(FILE).pdf
	$(RM) $(FILE).ps
	$(RM) $(FILE).dvi
	$(RM) *.d


==> sections/analysis.tex <==
\section{Latency Analysis} \label{sec:analysis}

\alberto{Do we want this section or do we integrate its content into related work and proofs? Discuss this once we have more graphs.}

\alberto{Fill this section with Igor's latency analysis.}
